The Age of Information: Real-Time Status Updating by Multiple Sources

We examine multiple independent sources providing status updates to a monitor through simple queues. We formulate an Age of Information (AoI) timeliness metric and derive a general result for the AoI that is applicable to a wide variety of multiple source service systems. For first-come first-served and two types of last-come first-served systems with Poisson arrivals and exponential service times, we find the region of feasible average status ages for multiple updating sources. We then use these results to characterize how a service facility can be shared among multiple updating sources. A new simplified technique for evaluating the AoI in finite-state continuous-time queueing systems is also derived. Based on stochastic hybrid systems, this method makes AoI evaluation to be comparable in complexity to finding the stationary distribution of a finite-state Markov chain.

==> mm1TwoSourcesLCFS.tex <==
% !TEX root =  TwoSourcesJournal.tex
%\section{M/M/1 Last-Come-First-Served}
%\label{sec:mm1LCFS}
%
%
%We defer the proof of \Thmref{LCFS} to Sections~\ref{sec:lcfsWithpre}, \ref{sec:lcfsWithpre-SHS} and~\ref{sec:lcfsWOpreMM1}.
%

%It appears that because \cite{2012CISS-KaulYatesGruteser} derived the result of \Thmref{LCFS}(a) (appearing as Equation~(47) in \cite{2012CISS-KaulYatesGruteser}) with a method similar to that used in \cite{2012CISS-KaulYatesGruteser} to derive an incorrect result, the authors in \cite{CostaCodreanuEphremides2016} have speculated that \Thmref{LCFS}(a) is also incorrect.





